Improving Contextual Recognition of Rare Words with an Alternate Spelling Prediction Model

Contextual ASR, which takes a list of bias terms as input along with audio, has drawn recent interest as ASR use becomes more widespread. We are releasing contextual biasing lists to accompany the Earnings21 dataset, creating a public benchmark for this task. We present baseline results on this benchmark using a pretrained end-to-end ASR model from the WeNet toolkit. We show results for shallow fusion contextual biasing applied to two different decoding algorithms. Our baseline results confirm observations that end-to-end models struggle in particular with words that are rarely or never seen during training, and that existing shallow fusion techniques do not adequately address this problem. We propose an alternate spelling prediction model that improves recall of rare words by 34.7% relative and of out-of-vocabulary words by 97.2% relative, compared to contextual biasing without alternate spellings. This model is conceptually similar to ones used in prior work, but is simpler to implement as it does not rely on either a pronunciation dictionary or an existing text-to-speech system.

==> notes.tex <==
Hybrid models:
\begin{itemize}
    \item G2P - is this in a paper somewhere?
    \item Composition-based on-the-fly rescoring for salient n-gram biasing \cite{hall2015composition}
    \item *** G2G: TTS-DRIVEN PRONUNCIATION LEARNING FOR GRAPHEMIC HYBRID ASR \cite{le2020g2g}
\end{itemize}

Shallow fusion (OTF rescoring) -- key thing to note here is that our approach can be combined with any/all of these
\begin{itemize}
    \item Contextual speech recognition in end-to-end neural network systems using beam search \cite{williams2018contextual} -- attention-based OTF
    \item End-to-end contextual speech recognition using class language models and a token passing decoder \cite{chen2019end} -- CLM not relevant to us
    \item Shallow-fusion end-to-end contextual biasing \cite{zhao2019shallow} -- testing lots of options, e.g. where does weight pushing happen
\end{itemize}

Deep biasing:
\begin{itemize}
    \item Deep context: end-to-end contextual speech recognition \cite{pundak2018deep} -- LAS model trained to also take embeddings of context words as input (CLAS)
    \item Phoebe: Pronunciation-aware contextualization for end-to-end speech recognition \cite{bruguier2019phoebe} -- builds on CLAS with option to input pronunciation info
    \item Joint grapheme and phoneme embeddings for contextual end-to-end ASR \cite{chen2019joint} -- another one that builds on CLAS
    \item Contextual speech recognition with difficult negative training examples \cite{alon2019contextual} -- another one!
    \item Contextual RNN-T for open domain ASR \cite{jain2020contextual} - CLAS for RNN-T
    \item Tree-Constrained Pointer Generator For End-To-End Contextual Speech Recognition \cite{sun2021tree} - this is the paper with the librispeech results. neurosymbolic model trained jointly with AED or RNN-T
\end{itemize}

Modifications to LM rescoring (shallow, but 2nd pass):
\begin{itemize}
    \item  Multi-Task Language Modeling For Improving Speech Recognition Of Rare Words \cite{yang2020multi}
    \item Contextualizing ASR lattice rescoring with hybrid pointer network language model \cite{liu2020contextualizing} - context comes from video descriptions
\end{itemize}

Other:
\begin{itemize}
    \item Remember The Context! Asr Slot Error Correction Through Memorization  \cite{bekal2021remember}
    \item Class LM and word mapping for contextual biasing in end-to-end ASR \cite{huang2020class} -- modification to training data to make class LM easier to use. *** also has pronunciation-based alternate spellings like we implemented! (ours is better but we can add those results to the paper)
    \item Hierarchical multi-stage word-to-grapheme named entity corrector for automatic speech recognition \cite{garg2020hierarchical} - named entity correction is maybe a whole separate field?
    \item "INSTANT ONE-SHOT WORD-LEARNING FOR CONTEXT-SPECIFIC NEURAL SEQUENCE-TO-SEQUENCE SPEECH RECOGNITION" \cite{huber2021instant}
    \item Fast and robust unsupervised contextual biasing for speech recognition \cite{kang2020fast}
\end{itemize}

Both shallow fusion + deep biasing:
\begin{itemize} 
    \item Deep shallow fusion for RNN-T personalization \cite{le2021deep} -- **** this is a follow-up from the original G2G paper, they're still doing G2G with TTS, though. also it's a statistical model similar to G2P
    \item Contextualized streaming end-to-end speech recognition with trie-based deep biasing and shallow fusion \cite{le2021contextualized} -- same group as above, still using same G2G model
\end{itemize}
